A Formal C Memory Model for Separation Logic

The core of a formal semantics of an imperative programming language is a memory model that describes the behavior of operations on the memory. Defining a memory model that matches the description of C in the C11 standard is challenging because C allows both high-level (by means of typed expressions) and low-level (by means of bit manipulation) memory accesses. The C11 standard has restricted the interaction between these two levels to make more effective compiler optimizations possible, on the expense of making the memory model complicated. We describe a formal memory model of the (non-concurrent part of the) C11 standard that incorporates these restrictions, and at the same time describes low-level memory operations. This formal memory model includes a rich permission model to make it usable in separation logic and supports reasoning about program transformations. The memory model and essential properties of it have been fully formalized using the Coq proof assistant.

==> lstcoq.tex <==
%=======================================================================
% Définit le style ssr Gallina pour les listings (Assia Mahboubi 2007)

\lstdefinelanguage{coq} {
% Comments may or not include Latex commands
texcl=false,

% Vernacular commands
morekeywords=[1]{
Section, Module, End, Require, Import, Export,
Variable, Variables, Parameter, Parameters, Axiom, Hypothesis, Hypotheses,
Notation, Local, Tactic, Reserved, Scope, Open, Close, Bind, Delimit,
Definition, Let, Ltac, Fixpoint, CoFixpoint, Add, Morphism, Relation,
Implicit, Arguments, Set, Unset, Contextual, Strict, Prenex, Implicits,
Inductive, CoInductive, Record, Structure, Canonical, Coercion,
Context, Class, Global, Instance, Program, Infix,
Theorem, Lemma, Corollary, Proposition, Fact, Remark, Example,
Proof, Goal, Save, Qed, Defined, Hint, Resolve, Rewrite, View,
Search, Show, Print, Printing, All, Graph, Projections, inside, outside},

% Gallina
morekeywords=[2]{forall, exists, exists2, fun, fix, cofix, struct,
      match, with, end, as, in, return, let, is, then,
      for, of, nosimpl},

% Sorts
morekeywords=[3]{Type, Prop},

% Various tactics, some are std Coq subsumed by ssr, for the manual purpose
morekeywords=[4]{
         pose, set, move, case, elim, apply, clear,
            hnf, intro, intros, generalize, rename, pattern, after,
	    destruct, induction, using, refine, inversion, injection,
         rewrite, congr, unlock, compute, field, fourier,
            replace, fold, unfold, change, cutrewrite, simpl,
         have, suff, wlog, suffices, without, loss, nat_norm,
            assert, cut, trivial, revert, bool_congr, nat_congr,
	 symmetry, transitivity, auto, split, left, right, autorewrite},        

% Terminators
morekeywords=[5]{
         by, done, exact, tauto, romega, omega,
         assumption, solve, contradiction, discriminate},


% Control
morekeywords=[6]{do, last, first, try, idtac, repeat},

% Comments delimiters, we do turn this off for the manual
comment=[s]{(*}{*)},

% Spaces are not displayed as a special character
showstringspaces=false,

% Size of tabulations
tabsize=3,							

% Case sensitivity
sensitive=true, 

% Automatic breaking of long lines
breaklines=true,

% Default style for listings
basicstyle=\ttfamily,

% Position of captions is bottom
captionpos=b,							

% Style for (listings') identifiers
identifierstyle={\ttfamily\color{black}},
% Note : highlighting of Coq identifiers is done through a new
% delimiter definition through an lstset at the begining of the
% document. Don't know how to do better.

% Style for declaration keywords
keywordstyle=[1]{\ttfamily\bfseries},


%Style for iterators
%keywordstyle=[6]{\ttfamily\color{dkpink}},

% Style for strings
stringstyle=\ttfamily,

% Style for comments
commentstyle=\ttfamily,
}


==> permissions/instances.tex <==
\subsection{Permissions as a separation algebra}
\label{section:separation_instances}

This section gives the full definitions of the separation algebras involved
in the construction of the \CHtwoO{} permission system
\(\perm \defined \lockable {\counter \Q} + \Q\).

The \emph{counting separation algebra over a separation algebra \(A\)} has
elements \(\pair x y\) with \(x \in \Q\) and \(y \in A\).
The rational number \(x\) counts the number of existence permissions
(\ie{} permissions that only allow pointer arithmetic) that have been handed
out.
Existence permissions themselves are elements \(\pair x \sepempty\) with
\(x < 0\).
To ensure that the counting separation algebra is closed under
\(\sepunionSym\) and preserves splittability, the counter \(x\) is a rational
number instead of an integer.

\begin{definition}
Given a separation algebra \(A\), the \emph{counting separation algebra
\(\counter A \defined \Q \times A\) over \(A\)} is defined as:
%
\begin{flalign*}
\sepvalid {\pair x y} \defined{}& \sepvalid y
	\land (\sepunmapped y \impl x \le 0)
	\land (\sepunshared y \impl 0 \le x)	\\
\sepempty \defined{}& \pair 0 \sepempty \\
\sepdisjoint {\pair x y} {\pair {x'} {y'}} \defined{}&
	\sepdisjoint y {y'}
	\begin{array}[t]{l}
	\land\ (\sepunmapped y \impl x \le 0)
	\land (\sepunmapped {y'} \impl x' \le 0) \\
	\land\ (\sepunshared {(\sepunion y {y'})}
		\impl 0 \le x + x')
	\end{array}\\
\sepunion {\pair x y} {\pair {x'} {y'}} \defined{}&
	\pair {x + x'} {\sepunion y {y'}} \\
\sepsplittable {\pair x y} \defined{}&
    \sepsplittable y
    \land (\sepunmapped y \impl x \le 0) \land (\sepunshared y \impl 0 \le x) \\
\sephalf {\pair x y} \defined{}& \pair {0.5 \cdot x} {\sephalf y} \\
\sepunmapped {\pair x y} \defined{}&
	\sepunmapped y \land x \le 0 \\
\sepunshared {\pair x y} \defined{}&
	\sepunshared y \land 0 \le x
\end{flalign*}
%The definitions of the omitted relations and operations are as expected.
\end{definition}

The \emph{lockable separation algebra} adds annotations
\(\{ \LLockedSym, \LUnlockedSym \}\) to account for whether a permission is
locked \(\LLockedSym\) or not \(\LUnlockedSym\).
Permissions that are locked have exclusive write ownership, and are thus
only disjoint from those that are \(\sepunmappedSym\).

\begin{definition}
Given a separation algebra \(A\), the \emph{lockable separation algebra
\(\lockable A \defined \{ \LLockedSym, \LUnlockedSym \} \times A\) over \(A\)}
is defined as:
%
\begin{align*}
\sepvalid {(\LUnlocked x)} \defined{}& \sepvalid x
	& \sepvalid {(\LLocked x)} \defined{}& \sepunshared x \\
\sepempty \defined{}& \LUnlocked \sepempty
	& \\
\sepdisjoint {\LUnlocked x} {\LUnlocked y} \defined{}& \sepdisjoint x y
	& \sepdisjoint {\LUnlocked x} {\LLocked y} \defined{}&
	\sepdisjoint x y \land \sepunmapped x \land \sepunshared y \\
\sepdisjoint {\LLocked x} {\LLocked y} \defined{}& \False 
	& \sepdisjoint {\LLocked x} {\LUnlocked y} \defined{}&
	\sepdisjoint x y \land \sepunshared x \land \sepunmapped y \\
\sepunion {\LUnlocked x} {\LUnlocked y} \defined{}&
	\LUnlocked {(\sepunion x y)}
	& \sepunion {\LUnlocked x} {\LLocked y} \defined{}
	& \LLocked {(\sepunion x y)} \\
%\sepunion {\LLocked x} {\LLocked y} \defined{}& \LLocked {(\sepunion x y)}
	&& \sepunion {\LLocked x} {\LUnlocked y} \defined{}
	& \LLocked {(\sepunion x y)} \\
\sepsplittable {(\LLocked x)} \defined{}& \False &
\sepsplittable {(\LUnlocked x)} \defined{}& \sepsplittable x \\
%\sephalf {(\LLocked x)} \defined{}& \LLocked {(\sephalf x)} & 
&&
\sephalf {(\LUnlocked x)} \defined{}& \LUnlocked {(\sephalf x)} \\
\sepunmapped {(\LLocked x)} \defined{}& \False &
\sepunmapped {(\LUnlocked x)} \defined{}& \sepunmapped x \\
\sepunshared {(\LLocked x)} \defined{}& \sepunshared x &
\sepunshared {(\LLocked x)} \defined{}& \sepunshared x
\end{align*}
%The definitions of the omitted relations and operations are as expected.
\end{definition}

The separation algebra structure on the sum is intuitively straightforward,
but technically subtle because the \(\sepempty\) elements have
to be \emph{identified}.
We achieve this by ensuring that only the \(\sepempty\) element of \(A\) in
\(A + B\) is used.

\begin{definition}
Given a separation algebras \(A\) and \(B\), the separation algebra on the sum
\(A + B\) is defined as:
%
\allowdisplaybreaks[1]
\begin{align*}
\sepvalid {\inl x} \defined{}& \sepvalid x
	& \sepvalid {\inr x} \defined{}& \sepvalid x \land x \neq \sepempty \\
\sepempty \defined{}& \inl \sepempty && \\
\sepdisjoint {\inl x} {\inl y} \defined{}& \sepdisjoint x y
	& \sepdisjoint {\inr x} {\inr y} \defined{}&
		\sepdisjoint x y \land x \neq \sepempty \land y \neq \sepempty \\
\sepdisjoint {\inl x} {\inr y} \defined{}&
	x = \sepempty \land \sepvalid y \land y \neq \sepempty
	& \sepdisjoint {\inr x} {\inl y} \defined{}&
		\sepvalid x \land x \neq \sepempty \land y = \sepempty \\
\sepunion {\inl x} {\inl y} \defined{}& \inl {(\sepunion x y)}
	& \sepunion {\inr x} {\inr y} \defined{}& \inr {(\sepunion x y)} \\
\sepunion {\inl x} {\inr y} \defined{}& \inr y
	& \sepunion {\inr x} {\inl y} \defined{}& \inr x \\
\sepsplittable {\inl x} \defined& \sepsplittable x
	& \sepsplittable {\inr x} \defined& \sepsplittable x \land x = \sepempty \\
\sephalf {(\inl x)} \defined& \inl{(\sephalf x)}
	& \sephalf {(\inr x)} \defined& \inr{(\sephalf x)} \\
\sepunmapped {\inl x} \defined{}& \sepunmapped x
	& \sepunmapped {\inr x} \defined{}& \sepunmapped x \land x \neq \sepempty \\
\sepunshared {\inl x} \defined{}& \sepunshared x
	& \sepunshared {\inr x} \defined{}& \sepunshared x
\end{align*}
%The definitions of the omitted relations and operations are as expected.
\end{definition}

\begin{definition}
The operations on the \CHtwoO{} permission system
\(\permkindSym : A \to \pkind\), \(\permlockSym, \permunlockSym : A \to A\)
and \(\permtoken : A\) are defined as:
%
\allowdisplaybreaks[3]
\begin{flalign*}
\permkind \gamma \defined{}&
	\begin{cases}
	\Some\Writable & \textnormal{if \(\gamma = \LUnlocked {\pair x 1}\)} \\
	\Some\Readable &
		\textnormal{if \(\gamma = \LUnlocked {\pair x y}\) with \(0 < y < 1\)
		or \(\gamma = x\)} \\
	\Some\Existing &
		\textnormal{if \(\gamma = \LUnlocked {\pair x 0}\) with \(x \neq 0\)} \\
	\Some\Locked &	\textnormal{if \(\gamma = \LLocked {\pair x y}\)} \\
	\None & \textnormal{otherwise}
	\end{cases} \\
\permlock \gamma \defined{}&
	\begin{cases}
	\LLocked {\pair x y} & \textnormal{if \(\gamma = \LUnlocked {\pair x y}\)} \\
	\gamma & \textnormal{otherwise}
	\end{cases} \\
\permunlock \gamma \defined{}&
	\begin{cases}
	\LUnlocked {\pair x y}& \textnormal{if \(\gamma = \LLocked {\pair x y}\)} \\
	\gamma & \textnormal{otherwise}
	\end{cases} \\
\permtoken \defined{}& \LUnlocked {\pair {-1} 0}
\end{flalign*}
\end{definition}

\begin{lemma}
The \CHtwoO{} permission system satisfies the following properties:
%
\newcommand{\provided}{&&\hspace{-13.5em}}
\begin{align*}
\permunlock {(\permlock x)} ={}& x\
   \provided
   \textnormal{if } \Some\Writable \subseteq \permkind x \\
\permkind {(\permlock x)} ={}& \Some\Locked
   \provided \textnormal{if } \Some\Writable \subseteq \permkind x \\
\permkind {\big(\sephalf x\big)} ={}&
   \begin{cases}
   \Some\Readable & \textnormal{if } \Some\Writable \subseteq \permkind x \\
   \permkind x & \textnormal{otherwise}
   \end{cases}\\
\permkind \permtoken ={}& \Some\Existing \\
\permkind {(\sepdifference x \permtoken)} ={}& \permkind x \\
\permkind {x_1} \subseteq{}& \permkind {x_2}
   \provided \textnormal{if \(\sepsubseteq {x_1} {x_2}\)}
\end{align*}
\end{lemma}



==> syntax.tex <==
\chapter{Syntax}

\allowdisplaybreaks[3]

\section{Operators}
\begin{flalign*}
%<*binopc>
\binOp_c \in \compop \inductive{}& \EqOp\separator\LeOp\separator\LtOp
%</binopc>
\\
%<*binopb>
\binOp_b \in \bitop \inductive{}& \AndOp\separator\OrOp\separator\XorOp
%</binopb>
\\
%<*binopa>
\binOp_a \in \arithop \inductive{}& \PlusOp\separator\MinusOp\separator
	\MultOp\separator \DivOp\separator\ModOp
%</binopa>
\\
%<*binops>
\binOp_s \in \shiftop \inductive{}& \ShiftLOp\separator\ShiftROp
%</binops>
\\
%<*binop>
\binOp \in \binop \inductive{}& \binOp_c \separator \binOp_b \separator
	\binOp_a \separator \binOp_s
%</binop>
\\
%<*unop>
\unOp \in \unop \inductive{}& \NegOp \separator \ComplOp \separator \NotOp
%</unop>
\\
%<*assign>
\alpha \in \assign \inductive{} &
	\Assign \separator \PreOp \binOp \separator \PostOp \binOp
%</assign>
\end{flalign*}

\section{Types}
\begin{flalign*}
k \in K \defined{}& \mbox{Set of integer ranks} \\
t \in \stag \defined{}& \mbox{Strings denoting struct/union names} \\
f \in \funname \defined{}& \mbox{Strings denoting of function names} \\
%<*signedness>
si \in \signedness \inductive{}& \Signed \separator \Unsigned
%</signedness>
\\
%<*inttype>
\itype\tau \in \inttype \inductive{}& \IntType {si} k
%</inttype>
\\
%<*basetype>
\btype\tau, \btype\sigma \in \basetype \inductive{}&
	\TInt{\itype\tau} \separator
	\TPtr {\ptype\tau} \separator
	\TVoid
%</basetype>
\\
%<*ptrtype>
\ptype\tau, \ptype\sigma \in \ptrtype \inductive{}&
	\TType \tau \separator
	\TAny \separator
	\TFun {\vec\tau} \tau
%</ptrtype>
\\
%<*type>
\tau, \sigma \in \type \inductive{}&
	\TBase{\btype\tau} \separator
	\TArray \tau n \separator
	\TStruct t \separator
	\TUnion t
%</type>
\\
%<*env>
\Gamma \in \env \defined{}&
	(\map \stag {\lst\type}) \mathrel\times \tag{types of struct/union fields} \\
	&
	(\map \funname {(\lst\type} \times \type)) \tag{types of functions}
%	\emptyset \separator
%	\einsert t {\vec\tau} \Gamma \separator
%	\einsert f {\pair {\vec\tau} \tau} \Gamma
%</env>
\end{flalign*}

\section{Permissions}
\begin{flalign*}
\lockable A \defined{}& \{ \LLockedSym, \LUnlockedSym \} \times A 
	\tag{lockable separation algebra}\\
\counter A \defined{}& \Q \times A \tag{counting separation algebra} \\
\tagged A t T \defined{}& A \times T \textnormal{ with }t \in T
	\tag{tagged separation algebra}\\
%<*perm>
\gamma \in \perm \defined{}& \lockable {\counter \Q} + \Q
%</perm>
\end{flalign*}

\section{Memory model}
\begin{flalign*}
o \in \memindex \defined{}& \mbox{Set of memory indices} \\
\Delta \in \memenv \defined{}& \map \memindex {(\type \times \bool)} \\
%<*refseg>
r \in \rrefseg \inductive{}&
	\RArray i \tau n \separator
	\RStruct i t \separator
	\RUnion i t q
	\textnormal{ with \(q \in \{ \RFrozen, \RUnfrozen \}\)}
%</refseg>
\\
%<*ref>
\vec r \in \rref \defined{}& \lst\rrefseg
%</ref>
\\
%<*addr>
a \in \addr \inductive{}& \Addr o \tau {\vec r} i \sigma {\ptype\sigma}
%</addr>
\\
%<*ptr>
p \in \ptr \inductive{}&
	\NULL {\ptype\sigma} \separator \Ptr a \separator \FunPtr f {\vec\tau} \tau
%</ptr>
\\
%<*bit>
b \in \bit \inductive{} &
	\BIndet \separator
	\BBit 0 \separator \BBit 1 \separator
	\BPtrSeg {\PtrSeg p i} 
%</bit>
\\
%<*pbit>
\ppbit b \in \pbit \defined{}& \tagged \perm \BIndet \bit
%</pbit>
\\
%<*mtree>
w \in \mtree \inductive{} &
	\MBase {\btype \tau} {\vec {\ppbit b}} \separator
	\MArray \tau {\vec w} \separator
	\MStruct t {\vv{w\vec {\ppbit b}}} \separator
	\MUnion t i w {\vec {\ppbit b}} \separator
	\MUnionAll t {\vec {\ppbit b}}
%</mtree>
\\
%<*mem>
m \in \mem \defined{}& \map \memindex {(\mtree \times \bool + \type)}
%</mem>
\\
%<*baseval>
\bval v \in \baseval \inductive{}&
	\VIndet {\btype \tau} \separator
	\VVoid \separator
	\VInt {\itype \tau} x \separator
	\VPtr p \separator
	\VByte {\vec b}
%</baseval>
\\
%<*val>
v \in \val \inductive{}&
	\VBase {\bval v} \separator
	\VArray \tau {\vec v} \separator
	\VStruct t {\vec v} \separator
	\VUnion t i v \separator
	\VUnionAll t {\vec v}
%</val>
\\
%<*lockset>
\Omega \in \lockset \defined{}& \finset {\memindex \times \nat}
%</lockset>
\end{flalign*}

\section{\coreC}
\begin{flalign*}
l \in \labelname \defined{}& \mbox{Strings denoting labels} \\
%<*lrval>
\nu \in \lrval \defined{}& \ptr + \val
%</lrval>
\\
%<*expr>
e \in \expr \inductive{}&
	\EVar i \separator
	\EVal \Omega \nu
		\tag{variables and constants} \\ & \separator
	\ERtoL e \separator
	\ERofL e
		\tag{l-value and r-value conversion} \\ & \separator
	\EEltL e r \separator
	\EEltR e r
		\tag{indexing of arrays, structs and unions}\\ & \separator
	\EInsert {\vec r} {e_2} {e_1}
		\tag{altering arrays, structs and unions}\\ & \separator
	\EAssign \alpha {e_1} {e_2} \separator
	\ELoad e
		\tag{assignments and loading from memory}\\ & \separator
	\ECall e {\vec e} \separator
	\EAbort \tau
		\tag{function calls and undefined behavior}\\ & \separator
	\EAlloc \tau e \separator
	\EFree e
		\tag{allocation and deallocation}\\ & \separator
	\EUnOp \unOp e \separator
	\EBinOp \binOp {e_1} {e_2} \separator
	\ECast \tau e
		\tag{unary, binary and cast operators} \\& \separator
	\EComma {e_1} {e_2} \separator
	\EIf {e_1} {e_2} {e_3} \tag{comma and sequenced conditional}
%</expr>
\\
%<*stmt>
s \in \stmt \inductive{}&
	\SDo e \separator
	\SReturn e
		\tag{expression and \creturn{} statements} \\ & \separator
	\SGoto l \separator
	\SLabel l
		\tag{\cgoto{} and label} \\ & \separator
	\SThrow n \separator
	\SCatch s
		\tag{\cthrow{} and \ccatch} \\ & \separator
	\SSkip \separator
	\SComp {s_1} {s_2}
		\tag{the skip statement and composition} \\ & \separator
	\SLocal \tau s
		\tag{block scope local variable declaration} \\ & \separator
	\SLoop s
		\tag{infinite loop} \\ & \separator
	\SIf e {s_1} {s_2}
		\tag{conditional statement}
%</stmt>
\\
%<*funenv>
\delta \in \funenv \defined{}& \map \funname \stmt
%</funenv>
\end{flalign*}

\section{\coreC{} states}
\begin{flalign*}
%<*ectxitem>
\eectxitem E \in \ectxitem \inductive{}&
	\CRtoL \separator
	\CRofL \separator
	\CEltL r \separator
	\CEltR r \separator
	\CInsertR {\vec r} {e_2} \separator
	\CInsertL {\vec r} {e_1} \\& \separator
	\CAssignL \alpha {e_2} \separator
	\CAssignR \alpha {e_1} \separator
	\CLoad \separator
	\CCallL {\vec e} \separator
	\CCallR e {\vec e_1} {\vec e_2} \separator
	\CAlloc \tau \separator 
	\CFree \\&  \separator
	\CUnOp \unOp \separator
	\CBinOpL \binOp {e_2} \separator
	\CBinOpR \binOp {e_1} \separator
	\CCast \tau \separator
	\CIf {e_2} {e_3} \separator
	\CComma {e_2}
%</ectxitem>
\\
%<*ectx>
\eectx E \in \ectx \defined{}& \lst\ectxitem
%</ectx>
\\
%<*sctxitem>
\ssctxitem S \in \sctxitem \inductive{}&
	\CCatch \separator
	\CCompL {s_2} \separator
	\CCompR {s_1} \separator
	\CLoop \separator
	\CIfL e {s_2} \separator
	\CIfR e {s_1}
%</sctxitem>
\\
%<*esctxitem>
\eesctxitem S \in \esctxitem \inductive{}&
	\CDoE \separator
	\CReturnE \separator
	\CIfE {s_1} {s_2}
%</esctxitem>
\\
%<*ctxitem>
\cctxitem P \in \ctxitem \inductive{}&
	\CStmt {\ssctxitem S} \separator
	\CLocal o \tau \separator
	\CExpr e {\eesctxitem S} \separator
	\CFun {\eectx E} \separator
	\CParams f {\vv {o\tau}}
%</ctxitem>
\\
%<*ctx>
	\cctx P \in \ctx \defined{}& \lst\ctxitem
%</ctx>
\\
%<*stack>
	\rho \in \stack \defined{}& \lst {(\memindex \times \type)}
%</stack>
\\
%<*direction>
d \in \direction \inductive{}&
	\DDown \separator
	\DUp \separator
	\DGoto l \separator
	\DThrow n \separator
	\DTop v
%</direction>
\\
%<*focus>
\phi_U \in \undefstate \inductive{}&
	\UndefExpr {\eectx E} e \separator
	\UndefBranch {\eesctxitem S} \Omega v \\
\phi \in \focus \inductive{}&
	\Stmt d s \separator
	\Expr e \separator
	\Call f {\vec v} \separator
	\Return f v \separator
	\Undef {\phi_U}
%</focus>
\\
%<*state>
S \in \state \inductive{}&
	\State {\cctx P} \phi m
%</state>
\end{flalign*}

\section{\abstractC}
\begin{flalign*}
x \in \sstring \defined{}& \textnormal{Set of strings} \\
%<*cinttype>
k \in \cintrank \inductive{}&
	\CCharRank \separator \CShortRank \separator \CIntRank \separator
	\CLongRank \separator \CLongLongRank \separator \CPtrRank \\
si \in \signedness \inductive{}& \Signed \separator \Unsigned \\
\itype\tau \in \cinttype \inductive{}& \CIntType {\opt {si}} k
%</cinttype>
\\
%<*cexpr>
\tau \in \ctype \inductive{}&
	\CTVoid \separator
	\CTDef x \separator
	\CTInt {\itype\tau} \separator
	\CTPtr \tau \separator
	\CTFun {\vv {\tau\,\opt x}} \tau \separator
	\CTArray \tau e \\ &\separator
	\CTStruct x \separator
	\CTUnion x \separator
	\CTEnum x \separator
	\CTTypeOf e \\
e \in \cexpr \inductive{}&
	\CEVar x \separator
	\CEConst {\itype\tau} z \separator
	\CEString {\vec z}
		\tag{variables, integer and string constants}\\ & \separator
	\CESizeOf \tau \separator
	\CEAlignOf \tau \separator
	\CEOffsetOf \tau x \\ & \separator
	\CEMin \tau \separator
	\CEMax \tau \separator
	\CEBits \tau
		\tag{implementation defined constants}\\ & \separator
	\CEAddrOf e \separator
	\CEDeref e
		\tag{address of and dereference operator}\\ & \separator
	\CEField e x
		\tag{indexing of structs and unions}\\ & \separator
	\CEAssign \alpha {e_1} {e_2}
		\tag{assignments}\\ & \separator
	\CECall e {\vec e} \separator
%	\CEAbort
		\tag{function calls}\\ & \separator
	\CEAlloc \tau e \separator
	\CEFree e
		\tag{allocation and deallocation}\\ & \separator
	\CEUnOp \unOp e \separator
	\CEBinOp \binOp {e_1} {e_2} \separator
	\CECast \tau I
		\tag{unary, binary and cast operators} \\& \separator
	\CEAnd {e_1} {e_2} \separator
	\CEOr {e_1} {e_2} \separator
	\CEComma {e_1} {e_2} \separator
	\CEIf {e_1} {e_2} {e_3}
	\tag{sequenced operators} \\
r \in \crefseg \inductive{}&
	\CRArray e \separator
	\CRcompound x \displaybreak[3] \\
I \in \cinit \inductive{}&
	\CSingleInit e \separator
	\CCompoundInit {\vv{\vv r := I}}
%</cexpr>
\\
%<*cstmt>
sto \in \cstorage \inductive{}&
	\StaticStorage \separator \ExternStorage \separator \AutoStorage \\
s \in \cstmt \inductive{}&
	\CSDo e \separator
	\CSReturn {\opt e}
		\tag{expression and \creturn{} statements} \\ & \separator
	\CSGoto x \separator
	\CSLabel x s
		\tag{\cgoto{} and label} \\ & \separator
	\CSBreak \separator
	\CSContinue
		\tag{\cbreak{} and \ccontinue} \\ & \separator
	\CSScope s
		\tag{block scope} \\ & \separator
	\CSLocal {\vv{sto}} x \tau {\opt I} s
		\tag{local variable declaration} \\ & \separator
	\CSTypeDef x \tau s
		\tag{local typedef declaration} \\ & \separator
	\CSSkip \separator
	\CSComp {s_1} {s_2}
		\tag{the skip statement and composition} \\ & \separator
	\CSWhile e s \separator
	\CSDoWhile s e
		\tag{\cwhile{} loops} \\ & \separator
	\CSFor {e_1} {e_2} {e_3} s
		\tag{\cfor{} loop} \\ & \separator
	\CSIf e {s_1} {s_2}
		\tag{conditional statement}
%</cstmt>
\\
%<*decl>
d \in \decl \inductive{}&
	\StructDecl {\vv {\tau\,x}} \separator
	\UnionDecl {\vv {\tau\,x}}
		\tag{struct and union declarations} \\ & \separator
	\EnumDecl {\itype\tau} {\vv {x := \opt e}}
		\tag{enum declaration} \\ & \separator
	\TypeDefDecl \tau
		\tag{global typedef declaration} \\ & \separator
	\GlobDecl {\vv{sto}} \tau {\opt I}
		\tag{global variable declaration} \\ & \separator
	\FunDecl {\vv{sto}} \tau s
		\tag{function declaration}
%</decl>
\\
%<*decls>
\Theta \in \decls \defined{}& \lst {(\sstring \times \decl)}
%</decls>
\end{flalign*}

